On the Bipartite Entanglement Capacity of Quantum Networks

We consider the problem of multi-path entanglement distribution to a pair of nodes in a quantum network consisting of devices with non-deterministic entanglement swapping capabilities. Multi-path entanglement distribution enables a network to establish end-to-end entangled links across any number of available paths with pre-established link-level entanglement. Probabilistic entanglement swapping, on the other hand, limits the amount of entanglement that is shared between the nodes; this is especially the case when, due to architectural and other practical constraints, swaps must be performed in temporal proximity to each other. Limiting our focus to the case where only bipartite entangled states are generated across the network, we cast the problem as an instance of generalized flow maximization between two quantum end nodes wishing to communicate. We propose a mixed-integer quadratically constrained program (MIQCP) to solve this flow problem for networks with arbitrary topology. We then compute the overall network capacity, defined as the maximum number of EPR states distributed to users per time unit, by solving the flow problem for all possible network states generated by probabilistic entangled link presence and absence, and subsequently by averaging over all network state capacities. The MIQCP can also be applied to networks with multiplexed links. While our approach for computing the overall network capacity has the undesirable property that the total number of states grows exponentially with link multiplexing capability, it nevertheless yields an exact solution that serves as an upper bound comparison basis for the throughput performance of easily-implementable yet non-optimal entanglement routing algorithms. We apply our capacity computation method to several networks, including a topology based on SURFnet -- a backbone network used for research purposes in the Netherlands.

==> Lemma1Proof.tex <==
%%!TEX PS-program = pdflatexmk
%%!TEX root = tqe.tex
\begin{proof}

Suppose $\sum_i x_{ijk} = 0$ for some edge $(j,k)$, and recall that $j\neq t$ (since by our definition of $G$, there are no outgoing edges from $t$). Assume for a contradiction that $F_{jk}>0$. Then from condition (\ref{eq:flowcons}) for node $j$, we can see that
\begin{align}
F_{jk}+\sum\limits_{i\neq k}F_{ji}-q_j\sum\limits_{i\in V}F_{ij}=0,
\label{eq:jflow1}
\end{align}
which implies that there exists some $\pr{i}$ such that $F_{\pr{i}j}>0$ (since if no such $\pr{i}$ exists, (\ref{eq:flowcons}) is violated due to the left-hand side being strictly positive). Thus, Eq. (\ref{eq:jflow1}) may be rewritten as
\begin{align}
F_{jk}+\sum\limits_{i\neq k}F_{ji}-q_jF_{\pr{i}j}-q_j\sum\limits_{i\neq \pr{i}}F_{ij}=0.
\label{eq:jflow2}
\end{align}
Note that it is possible that $\pr{i}=k$.
The case of $\pr{i}\neq k$ is depicted in Figure \ref{fig:EX1}, although the proof is the same even if $\pr{i}=k$. Since $F_{\pr{i}j}>0$, by condition (\ref{eq:xflow2}) there must be some $l$ such that $x_{\pr{i}jl}=1$, and by condition (\ref{eq:xijk3}), this $l$ is unique. Further, by definition of $x_{ijk}$ variables, $l\neq \pr{i}$, $l\neq j$, and by our assumption that $\sum_i x_{ijk} = 0$, it follows that $x_{\pr{i}jk}=0$ so that $l\neq k$. Also, by condition (\ref{eq:xflow1}), we must have
\begin{align}
F_{\pr{i}j}q_j = F_{jl},
\label{eq:jflow3}
\end{align}
which implies that $F_{jl}$ is strictly positive. This is depicted in Figure \ref{fig:EX2}. Since $l\neq k$, it must be in the first sum of Eq. (\ref{eq:jflow2}), and we may write
\begin{align*}
F_{jk}+F_{jl}+\sum\limits_{i\neq k,l}F_{ji}-q_jF_{\pr{i}j}-q_j\sum\limits_{i\neq \pr{i}}F_{ij}=0,
\end{align*}
and by Eq. (\ref{eq:jflow3}),
\begin{align}
F_{jk}+\sum\limits_{i\neq k,l}F_{ji}-q_j\sum\limits_{i\neq \pr{i}}F_{ij}=0.
\label{eq:jflow4}
\end{align}
Comparing Eqs. (\ref{eq:jflow1}) and (\ref{eq:jflow4}), we see that the only difference is that in the latter, two components on the left-hand side have cancelled each other out: one from each of the sums, while the $F_{jk}$ component has not changed at all. If we now attempt to balance out $F_{jk}$ using another (negative) component from the second sum above, say $F_{i^{\prime\prime}j}$, we ensure by conditions (\ref{eq:xflow2}) and (\ref{eq:xijk3}) the existence of a unique $n$ for which $x_{i^{\prime\prime}jn}=1$, and by condition (\ref{eq:xflow1}) enforce the strict positivity of $F_{jn}$. Note that since $x_{\pr{i}jl}=1$, we cannot also have $x_{i^{\prime\prime}jl}=1$ (condition (\ref{eq:xijk3})), which means that $n \neq l$. Finally, $n \neq k$ since if it were, then $x_{\pr{i}jk}$ would be equal to one, but $\sum\limits_{i}x_{ijk}=0$ by our assumption. Thus, any time we attempt to balance out $F_{jk}$ with a negative component from Eq. (\ref{eq:flowcons}), we force another flow into node $k$ to be strictly positive, and this positive flow cancels the negative component, leaving $F_{jk}$ unaffected. We can continue this cancellation process until there are no longer any negative components left in the flow balance equation, which would leave us with a strictly positive value on the left-hand side that is $\geq F_{jk}$. From this, we conclude that $\sum\limits_{i}x_{ijk}=0 \implies F_{jk} =0$.
\end{proof}

==> tqe.bbl_16.05.58 <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{munro2015inside}
W.~J. Munro, K.~Azuma, K.~Tamaki, and K.~Nemoto, ``Inside quantum repeaters,''
  \emph{IEEE Journal of Selected Topics in Quantum Electronics}, vol.~21,
  no.~3, pp. 78--90, 2015.

\bibitem{muralidharan2016optimal}
S.~Muralidharan, L.~Li, J.~Kim, N.~L{\"u}tkenhaus, M.~D. Lukin, and L.~Jiang,
  ``Optimal architectures for long distance quantum communication,''
  \emph{Scientific reports}, vol.~6, no.~1, pp. 1--10, 2016.

\bibitem{bennet1984quantum}
C.~H. Bennett and G.~Brassard, ``Quantum cryptography: Public key distribution
  and coin tossing,'' in \emph{Proceedings of the IEEE International Conference
  on Computers, Systems, and Signal Processing, Bangalore, Dec. 1984}, 1984,
  pp. 175--179.

\bibitem{ekert1991quantum}
A.~K. Ekert, ``{Quantum cryptography based on Bell’s theorem},''
  \emph{Physical review letters}, vol.~67, no.~6, p. 661, 1991.

\bibitem{bennett1992quantum}
C.~H. Bennett, G.~Brassard, and N.~D. Mermin, ``{Quantum cryptography without
  Bell’s theorem},'' \emph{Physical review letters}, vol.~68, no.~5, p. 557,
  1992.

\bibitem{broadbent2009universal}
A.~Broadbent, J.~Fitzsimons, and E.~Kashefi, ``Universal blind quantum
  computation,'' in \emph{2009 50th Annual IEEE Symposium on Foundations of
  Computer Science}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2009, pp.
  517--526.

\bibitem{leichtle2021verifying}
D.~Leichtle, L.~Music, E.~Kashefi, and H.~Ollivier, ``Verifying bqp
  computations on noisy devices with minimal overhead,'' \emph{PRX Quantum},
  vol.~2, no.~4, p. 040302, 2021.

\bibitem{duan2001long}
L.-M. Duan, M.~D. Lukin, J.~I. Cirac, and P.~Zoller, ``Long-distance quantum
  communication with atomic ensembles and linear optics,'' \emph{Nature}, vol.
  414, no. 6862, pp. 413--418, 2001.

\bibitem{maier2020investigating}
D.~Maier, ``Investigating the scalability of quantum repeater protocols based
  on atomic ensembles,'' Master's thesis, 2020.

\bibitem{rabbie2020simulation}
J.~Rabbie, ``Simulation model for atomic ensemble based quantum repeaters and
  the optimization of their positioning,'' Master's thesis, 2020.

\bibitem{caleffi2017optimal}
M.~Caleffi, ``Optimal routing for quantum networks,'' \emph{IEEE Access},
  vol.~5, pp. 22\,299--22\,312, 2017.

\bibitem{van2013path}
R.~Van~Meter, T.~Satoh, T.~D. Ladd, W.~J. Munro, and K.~Nemoto, ``Path
  selection for quantum repeater networks,'' \emph{Networking Science}, vol.~3,
  pp. 82--95, 2013.

\bibitem{gyongyosi2017entanglement}
L.~Gyongyosi and S.~Imre, ``Entanglement-gradient routing for quantum
  networks,'' \emph{Scientific reports}, vol.~7, no.~1, pp. 1--14, 2017.

\bibitem{schoute2016shortcuts}
E.~Schoute, L.~Mancinska, T.~Islam, I.~Kerenidis, and S.~Wehner, ``Shortcuts to
  quantum network routing,'' \emph{arXiv preprint arXiv:1610.05238}, 2016.

\bibitem{gyongyosi2018decentralized}
L.~Gyongyosi and S.~Imre, ``Decentralized base-graph routing for the quantum
  internet,'' \emph{Physical Review A}, vol.~98, no.~2, p. 022310, 2018.

\bibitem{chakraborty2019distributed}
K.~Chakraborty, F.~Rozpedek, A.~Dahlberg, and S.~Wehner, ``Distributed routing
  in a quantum internet,'' \emph{arXiv preprint arXiv:1907.11630}, 2019.

\bibitem{pirandola2019end}
S.~Pirandola, ``End-to-end capacities of a quantum communication network,''
  \emph{Communications Physics}, vol.~2, no.~1, p.~51, 2019.

\bibitem{azuma2016fundamental}
K.~Azuma, A.~Mizutani, and H.-K. Lo, ``{Fundamental rate-loss trade-off for the
  quantum internet},'' \emph{Nature communications}, vol.~7, no.~1, p. 13523,
  2016.

\bibitem{harney2022end}
C.~Harney and S.~Pirandola, ``{End-to-end capacities of imperfect-repeater
  quantum networks},'' \emph{Quantum Science and Technology}, vol.~7, no.~4, p.
  045009, 2022.

\bibitem{azuma2017aggregating}
K.~Azuma and G.~Kato, ``{Aggregating quantum repeaters for the quantum
  internet},'' \emph{Physical Review A}, vol.~96, no.~3, p. 032332, 2017.

\bibitem{bauml2020linear}
S.~B{\"a}uml, K.~Azuma, G.~Kato, and D.~Elkouss, ``{Linear programs for
  entanglement and key distribution in the quantum internet},''
  \emph{Communications Physics}, vol.~3, no.~1, p.~55, 2020.

\bibitem{dai2020optimal}
W.~Dai, T.~Peng, and M.~Z. Win, ``Optimal remote entanglement distribution,''
  \emph{IEEE Journal on Selected Areas in Communications}, vol.~38, no.~3, pp.
  540--556, 2020.

\bibitem{cicconetti2021request}
C.~Cicconetti, M.~Conti, and A.~Passarella, ``Request scheduling in quantum
  networks,'' \emph{IEEE Transactions on Quantum Engineering}, vol.~2, pp.
  2--17, 2021.

\bibitem{le2022dqra}
L.~Le and T.~N. Nguyen, ``{DQRA: Deep Quantum Routing Agent for Entanglement
  Routing in Quantum Networks},'' \emph{IEEE Transactions on Quantum
  Engineering}, vol.~3, pp. 1--12, 2022.

\bibitem{victora2020purification}
M.~Victora, S.~Tserkis, S.~Krastanov, A.~S. de~la Cerda, S.~Willis, and
  P.~Narang, ``Entanglement purification on quantum networks,'' \emph{Physical
  Review Research}, vol.~5, no.~3, Sep. 2023.

\bibitem{yang2022online}
L.~Yang, Y.~Zhao, H.~Xu, and C.~Qiao, ``Online entanglement routing in quantum
  networks,'' in \emph{2022 IEEE/ACM 30th International Symposium on Quality of
  Service (IWQoS)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2022, pp.
  1--10.

\bibitem{nguyen2022multiple}
T.~N. Nguyen, K.~J. Ambarani, L.~Le, I.~Djordjevic, and Z.-L. Zhang, ``A
  multiple-entanglement routing framework for quantum networks,'' \emph{arXiv
  preprint arXiv:2207.11817}, 2022.

\bibitem{zeng2022multi}
Y.~Zeng, J.~Zhang, J.~Liu, Z.~Liu, and Y.~Yang, ``Multi-entanglement routing
  design over quantum networks,'' in \emph{IEEE INFOCOM 2022 - IEEE Conference
  on Computer Communications}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, May
  2022.

\bibitem{zhang2022multipath}
L.~Zhang, S.-X. Ye, Q.~Liu, and H.~Chen, ``Multipath concurrent entanglement
  routing in quantum networks based on virtual circuit,'' in \emph{2022 4th
  International Conference on Advances in Computer Technology, Information
  Science and Communications (CTISC)}.\hskip 1em plus 0.5em minus 0.4em\relax
  IEEE, 2022, pp. 1--5.

\bibitem{nguyen2022maximizing}
T.~N. Nguyen, D.~H. Nguyen, D.~H. Pham, B.-H. Liu, and H.~N. Nguyen, ``{LP
  Relaxation-Based Approximation Algorithms for Maximizing Entangled Quantum
  Routing Rate},'' in \emph{ICC 2022-IEEE International Conference on
  Communications}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2022, pp.
  3269--3274.

\bibitem{amer2020efficient}
O.~Amer, W.~O. Krawec, and B.~Wang, ``Efficient routing for quantum key
  distribution networks,'' in \emph{2020 IEEE International Conference on
  Quantum Computing and Engineering (QCE)}.\hskip 1em plus 0.5em minus
  0.4em\relax IEEE, 2020, pp. 137--147.

\bibitem{zhao2021redundant}
Y.~Zhao and C.~Qiao, ``Redundant entanglement provisioning and selection for
  throughput maximization in quantum networks,'' in \emph{IEEE INFOCOM
  2021-IEEE Conference on Computer Communications}.\hskip 1em plus 0.5em minus
  0.4em\relax IEEE, 2021, pp. 1--10.

\bibitem{ghaderibaneh2022pre}
M.~Ghaderibaneh, H.~Gupta, C.~Ramakrishnan, and E.~Luo, ``Pre-distribution of
  entanglements in quantum networks,'' in \emph{2022 IEEE International
  Conference on Quantum Computing and Engineering (QCE)}.\hskip 1em plus 0.5em
  minus 0.4em\relax IEEE, 2022, pp. 426--436.

\bibitem{li2022fidelity}
J.~Li, M.~Wang, K.~Xue, R.~Li, N.~Yu, Q.~Sun, and J.~Lu, ``Fidelity-guaranteed
  entanglement routing in quantum networks,'' \emph{IEEE Transactions on
  Communications}, vol.~70, no.~10, pp. 6748--6763, 2022.

\bibitem{li2021effective}
C.~Li, T.~Li, Y.-X. Liu, and P.~Cappellaro, ``Effective routing design for
  remote entanglement generation on quantum networks,'' \emph{npj Quantum
  Information}, vol.~7, no.~1, pp. 1--12, 2021.

\bibitem{shi2020concurrent}
S.~Shi and C.~Qian, ``Concurrent entanglement routing for quantum networks:
  Model and designs,'' in \emph{Proceedings of the Annual conference of the ACM
  Special Interest Group on Data Communication on the applications,
  technologies, architectures, and protocols for computer communication}, 2020,
  pp. 62--75.

\bibitem{chakraborty2020entanglement}
K.~Chakraborty, D.~Elkouss, B.~Rijsman, and S.~Wehner, ``Entanglement
  distribution in a quantum network: A multicommodity flow-based approach,''
  \emph{IEEE Transactions on Quantum Engineering}, vol.~1, pp. 1--21, 2020.

\bibitem{pant2019routing}
M.~Pant, H.~Krovi, D.~Towsley, L.~Tassiulas, L.~Jiang, P.~Basu, D.~Englund, and
  S.~Guha, ``Routing entanglement in the quantum internet,'' \emph{npj Quantum
  Information}, vol.~5, no.~1, pp. 1--9, 2019.

\bibitem{patil2022entanglement}
A.~Patil, M.~Pant, D.~Englund, D.~Towsley, and S.~Guha, ``Entanglement
  generation in a quantum network at distance-independent rate,'' \emph{npj
  Quantum Information}, vol.~8, no.~1, p.~51, 2022.

\bibitem{leone2021qunet}
H.~Leone, N.~R. Miller, D.~Singh, N.~K. Langford, and P.~P. Rohde, ``Qunet:
  Cost vector analysis \& multi-path entanglement routing in quantum
  networks,'' \emph{arXiv preprint arXiv:2105.00418}, 2021.

\bibitem{acin2007entanglement}
A.~Ac{\'\i}n, J.~I. Cirac, and M.~Lewenstein, ``Entanglement percolation in
  quantum networks,'' \emph{Nature Physics}, vol.~3, no.~4, pp. 256--259, 2007.

\bibitem{skrzypczyk2021architecture}
M.~Skrzypczyk and S.~Wehner, ``{An Architecture for Meeting Quality-of-Service
  Requirements in Multi-User Quantum Networks},'' \emph{arXiv preprint
  arXiv:2111.13124}, 2021.

\bibitem{pompili2021experimental}
M.~Pompili, C.~Delle~Donne, I.~te~Raa, B.~van~der Vecht, M.~Skrzypczyk,
  G.~Ferreira, L.~de~Kluijver, A.~J. Stolk, S.~L. Hermans, P.~Pawe{\l}czak
  \emph{et~al.}, ``Experimental demonstration of entanglement delivery using a
  quantum network stack,'' \emph{npj Quantum Information}, vol.~8, no.~1, p.
  121, 2022.

\bibitem{kozlowski2019towards}
W.~Kozlowski and S.~Wehner, ``Towards large-scale quantum networks,'' in
  \emph{Proceedings of the Sixth Annual ACM International Conference on
  Nanoscale Computing and Communication}, 2019, pp. 1--7.

\bibitem{emilyTMPaper}
E.~A. Van~Milligen, E.~Jacobson, A.~Patil, G.~Vardoyan, D.~Towsley, and
  S.~Guha, ``{Entanglement Routing over Networks with Time Multiplexed
  Repeaters},'' \emph{arXiv preprint arXiv:2308.15028}, 2023.

\bibitem{gurobi}
\BIBentryALTinterwordspacing
{Gurobi Optimization, LLC}, ``{Gurobi Optimizer Reference Manual},'' 2023.
  [Online]. Available: \url{https://www.gurobi.com}
\BIBentrySTDinterwordspacing

\bibitem{github_repo}
\BIBentryALTinterwordspacing
G.~Vardoyan, ``Quantum network capacity,'' 2023. [Online]. Available:
  \url{https://github.com/gvardoyan/QuantumNetworkCapacity}
\BIBentrySTDinterwordspacing

\bibitem{ghose2005multihop}
S.~Ghose, R.~Kumar, N.~Banerjee, and R.~Datta, ``{Multihop virtual topology
  design in WDM optical networks for self-similar traffic},'' \emph{Photonic
  Network Communications}, vol.~10, no.~2, pp. 199--214, 2005.

\bibitem{rabbie2022designing}
J.~Rabbie, K.~Chakraborty, G.~Avis, and S.~Wehner, ``Designing quantum networks
  using preexisting infrastructure,'' \emph{npj Quantum Information}, vol.~8,
  no.~1, pp. 1--12, 2022.

\bibitem{repalloc}
\BIBentryALTinterwordspacing
J.~Rabbie and G.~Avis, ``{RepAlloc},'' 2020. [Online]. Available:
  \url{https://github.com/jtrabbie/RepAlloc}
\BIBentrySTDinterwordspacing

\bibitem{cabrillo1999creation}
C.~Cabrillo, J.~I. Cirac, P.~Garcia-Fernandez, and P.~Zoller, ``Creation of
  entangled states of distant atoms by interference,'' \emph{Physical Review
  A}, vol.~59, no.~2, p. 1025, 1999.

\bibitem{humphreys2018deterministic}
P.~C. Humphreys, N.~Kalb, J.~P. Morits, R.~N. Schouten, R.~F. Vermeulen, D.~J.
  Twitchen, M.~Markham, and R.~Hanson, ``Deterministic delivery of remote
  entanglement on a quantum network,'' \emph{Nature}, vol. 558, no. 7709, pp.
  268--273, 2018.

\end{thebibliography}

